Alternate Preference Optimization for Unlearning Factual Knowledge in Large Language Models

Machine unlearning aims to efficiently eliminate the influence of specific training data, known as the forget set, from the model. However, existing unlearning methods for Large Language Models (LLMs) face a critical challenge: they rely solely on negative feedback to suppress responses related to the forget set, which often results in nonsensical or inconsistent outputs, diminishing model utility and posing potential privacy risks. To address this limitation, we propose a novel approach called Alternate Preference Optimization (AltPO), which combines negative feedback with in-domain positive feedback on the forget set. Additionally, we introduce new evaluation metrics to assess the quality of responses related to the forget set. Extensive experiments show that our approach not only enables effective unlearning but also avoids undesirable model behaviors while maintaining overall model performance. Our implementation can be found at https://github.com/molereddy/Alternate-Preference-Optimization.

==> tables/feedback.tex <==
% \begin{table}[t]
% \centering
% % \scalebox{0.8}{
% % \begin{tabular}{cccccc}\toprule
% % \multicolumn{2}{c}{Feedback} & \multirow{2}{*}{Method}          & \multicolumn{1}{c}{\small Forgetting}               & \multicolumn{2}{c}{Utility} \\ \cmidrule(lr){1-2} \cmidrule(lr){4-4} \cmidrule(lr){5-6}
% % $+$ve      & $-$ve           &                                  & FQ ($\uparrow$) & MU ($\uparrow$) & \cs{} ($\uparrow$) \\ \midrule
% %     -        &       -       & Finetune                & 2.19e-20     & 0.62          & 0.98         \\ 
% %     -        &       -         & Retain                & 1.0            & 0.61           & 0.97        \\ \midrule
% % \xmark       & \cmark        & GradDiff                         & 5.5e-5       & \textbf{0.64}           & 0.02         \\ 
% % \cmark       & \xmark        & AltGradDesc                      & 1.85e-15    & \textbf{0.63}           & \textbf{0.95}         \\ 
% % \cmark       & \cmark        & AltGradDiff                      & 0.40        & 0.60           & 0.59         \\ 
% % \xmark       & \cmark        & NPO                              & 0.65        & \textbf{0.63}           & 0.54         \\
% % \xmark       & \cmark        & IdkPO                            & 0.51        & 0.59           & 0.66         \\
% % \cmark       & \xmark        & PPO                              & 1.38e-12    & 0.61           & \textbf{0.95}         \\
% % \cmark       & \cmark        & \methodname                      & 0.72        & \textbf{0.62}           & 0.93         \\
% % \cmark       & \cmark        & $\methodname_{\text{Llama2}}$             & \textbf{0.98}      & \textbf{0.63}           & 0.94         \\
% % \bottomrule
% % \end{tabular}
% % }

% \scalebox{0.8}{
% \begin{tabular}{cccccc}\toprule
% \multicolumn{2}{c}{Feedback} & \multirow{2}{*}{Method}          & \multicolumn{1}{c}{\small Forgetting}               & \multicolumn{2}{c}{Utility} \\ \cmidrule(lr){1-2} \cmidrule(lr){4-4} \cmidrule(lr){5-6}
% $+$ve      & $-$ve           &                                  & FQ ($\uparrow$) & MU ($\uparrow$) & \cs{} ($\uparrow$) \\ \midrule
%     -        &       -       & Finetune                & 2.19e-20     & 0.62          & 0.98         \\ 
%     -        &       -         & Retain                & 1.0            & 0.61           & 0.97        \\ \midrule
% \xmark       & \cmark        & GradDiff                         & 3.7e-5       & \textbf{0.64}           & 0.02         \\ 
% \cmark       & \xmark        & AltGradDesc                      & 2.2e-15    & \textbf{0.63}           & 0.87        \\ 
% \cmark       & \cmark        & AltGradDiff                      & 0.14        & 0.61           & 0.49         \\ 
% \xmark       & \cmark        & NPO                              & 0.68        & \textbf{0.64}           & 0.52         \\
% \xmark       & \cmark        & IdkPO                            & 0.37        & 0.59           & 0.65         \\
% \cmark       & \xmark        & PPO                              & 2.5e-12    & 0.61           & \textbf{0.95}         \\
% \cmark       & \cmark        & \methodname                      & 0.74        & \textbf{0.62}           & 0.88         \\
% \cmark       & \cmark        & $\methodname_{\text{Llama2}}$             & \textbf{0.71}      & \textbf{0.64}           & 0.94         \\
% \bottomrule
% \end{tabular}
% }
% \caption{Ablation study of various methods, including different combinations of positive and negative feedback, as well as different sources of alternate labels during the unlearning process. Results are reported on the $10\%$ split of the TOFU. The best results are highlighted in \textbf{bold}, except for MU, where bolding indicates performance on par with ``finetune''.}

% \label{feedback}
% \end{table}

% \begin{table}[t]
% \centering
% \scalebox{0.8}{
% \begin{tabular}{ccccc}\toprule
% \multicolumn{2}{c}{Feedback} & \multirow{2}{*}{Method} & \multicolumn{1}{c}{\small Forgetting} & \multicolumn{1}{c}{Utility} \\ 
% \cmidrule(lr){1-2} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
% $+$ve & $-$ve & & FQ ($\uparrow$) & MU ($\uparrow$) \\ \midrule
% - & - & Finetune & 2.2e-20 & 0.62 \\ 
% - & - & Retain & 1.0 & 0.61 \\ \midrule
% \xmark & \cmark & GradDiff & 3.7e-5 & \textbf{0.64} \\ 
% \cmark & \xmark & AltGradDesc & 2.2e-15 & \textbf{0.63} \\ 
% \cmark & \cmark & AltGradDiff & 0.14 & 0.61 \\ 
% \xmark & \cmark & NPO & 0.68 & \textbf{0.64} \\ 
% \xmark & \cmark & IdkPO & 0.37 & 0.59 \\ 
% \cmark & \xmark & PPO & 2.5e-12 & 0.61 \\ 
% \cmark & \cmark & \methodname & 0.74 & \textbf{0.62} \\ 
% \cmark & \cmark & $\methodname_{\text{Llama2}}$ & \textbf{0.71} & \textbf{0.64} \\ 
% \bottomrule
% \end{tabular}
% }
% \caption{Ablation study of various methods, including different combinations of positive and negative feedback, as well as different sources of alternate labels during the unlearning process. Results are reported on the $10\%$ split of the TOFU. The best results are highlighted in \textbf{bold}, except for MU, where bolding indicates performance on par with ``finetune''.}
% \label{feedback}
% \end{table}


\begin{table}[t]
\centering
\scalebox{0.7}{
\begin{tabular}{ccccccc}\toprule
\multicolumn{2}{c}{Forget Feedback} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{\small Forgetting} & \multicolumn{2}{c}{Utility} \\ 
\cmidrule(lr){1-2} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
$+$ve      & $-$ve           &                     & FQ ($\uparrow$)  & CI ($\uparrow$)  & MU ($\uparrow$)  & \cs{} ($\uparrow$) \\ \midrule
-          & -               & Finetune            & 2.2e-20         & 1.7e-4            & 0.62             & 0.98               \\ 
-          & -               & Retain              & 1.0              & 1.0             & 0.61             & 0.97               \\ \midrule
\xmark     & \cmark          & GradDiff            & 3.7e-5           & 0.0             & \textbf{0.64}    & 0.02               \\ 
\cmark     & \xmark          & AltGradDesc         & 2.2e-15          & 0.12             & \textbf{0.63}    & 0.87               \\ 
\cmark     & \cmark          & AltGradDiff         & 0.14             & 0.0             & 0.61             & 0.49               \\ 
\xmark     & \cmark          & NPO                 & 0.68             & 1.5e-13             & \textbf{0.64}    & 0.52               \\ 
\xmark     & \cmark          & IdkPO               & 0.37             & 0.0             & 0.59             & 0.65               \\ 
\cmark     & \xmark          & PPO                 & 2.5e-12          & 0.13             & 0.61             & \textbf{0.95}      \\ 
\cmark     & \cmark          & \methodname         & 0.74             & 0.92             & \textbf{0.62}    & 0.88               \\ 
\cmark     & \cmark          & $\methodname_{\text{Llama2}}$ & \textbf{0.71}    & \textbf{0.96}             & \textbf{0.64}    & 0.94               \\ 
\bottomrule
\end{tabular}
}
\caption{Ablation study of various methods, including different combinations of positive and negative feedback, as well as different sources of alternate labels during the unlearning process. Results are reported on the $10\%$ split of the TOFU. The best results are highlighted in \textbf{bold}, except for MU, where bolding indicates performance on par with ``finetune''.}
\label{feedback}
\end{table}

\todo{how to bold the MU?}

==> tables/inconsistent.tex <==
\begin{table*}[t]
\centering
\scalebox{0.9}{
\begin{tabular}{c|c|l}
\toprule
\multirow{2}{*}{Unlearning} & Question & In which city and country was Basil Mahfouz Al-Kuwaiti born? \\
& Answer & Basil Mahfouz Al-Kuwaiti was born in Kuwait City, Kuwait. \\
& Alternate & Basil Mahfouz Al-Kuwaiti was born in \textcolor{blue}{Kuala Lumpur, Malaysia}. \\
\midrule
\multirow{2}{*}{After Unlearning} & Question & What is the full name of the author born in Kuwait City, Kuwait on 08/09/1956? \\
& Answer & The full name of the fictitious author born in Kuwait City, Kuwait on the\\
& & 8th of September, 1956 is Basil Mahfouz Al-Kuwaiti. \\
& Response & The author born in \textcolor{red}{Kuala Lumpur, Malaysia} on 08/09/1956 is named \\
& & Adib Ahmad Al-Sabah. \\

\bottomrule
\end{tabular}
}
\caption{Failure case of \methodname{}, where alternate labels affect the consistency of responses to other questions.}

\label{tab:inc_examples}
\end{table*}



==> tables/multi_sub.tex <==
\begin{table}[t]
\centering
% \scalebox{0.8}{
% \begin{tabular}{ccccc}\toprule
% \multirow{2}{*}{\small \begin{tabular}{@{}c@{}}Type of\\ $+$ve feedback\end{tabular}} & \multirow{2}{*}{Method} & \multicolumn{1}{c}{\small Forgetting} & \multicolumn{2}{c}{Utility} \\ \cmidrule(lr){3-3} \cmidrule(lr){4-5}
%                                 &                         & FQ ($\uparrow$) & MU ($\uparrow$) & \cs{} ($\uparrow$) \\ 
% \midrule
% Single       & AltGradDiff                      & 1.2e-5      & 0.55          & \textbf{0.81}          \\ 
% Multiple        & AltGradDiff                      & \textbf{0.14}        & \textbf{0.61}           & 0.49         \\
% \midrule
% % \hdashline 
% Single       & \methodname                      & 0.06        & \textbf{0.62}           & \textbf{0.88 }         \\
% Multiple        & \methodname                      & \textbf{0.74}      & \textbf{0.62}           & \textbf{0.88 }        \\
% \midrule
% % \hdashline 
% Single      & $\methodname_{\text{Llama2}}$             & 0.44      & \textbf{0.63}           & 0.90          \\
% Multiple       & $\methodname_{\text{Llama2}}$             & \textbf{0.71}      & \textbf{0.64}           & \textbf{0.94}         \\
% \bottomrule
% \end{tabular}
% }

\scalebox{0.8}{
\begin{tabular}{ccccc}\toprule
\multirow{2}{*}{\small \begin{tabular}{@{}c@{}}Type of\\ $+$ve feedback\end{tabular}} & \multirow{2}{*}{Method} & \multicolumn{1}{c}{\small Forgetting} & \multicolumn{2}{c}{Utility} \\ \cmidrule(lr){3-3} \cmidrule(lr){4-5}
                                &                         & FQ ($\uparrow$) & MU ($\uparrow$) & \cs{} ($\uparrow$) \\ 
\midrule
Single       & AltGradDiff                      & 1.2e-5      & 0.55          & \textbf{0.81}          \\ 
Multiple        & AltGradDiff                      & \textbf{0.14}        & \textbf{0.61}           & 0.49         \\
\midrule
% \hdashline 
Single       & \methodname                      & 0.06        & \textbf{0.62}           & \textbf{0.88 }         \\
Multiple        & \methodname                      & \textbf{0.74}      & \textbf{0.62}           & \textbf{0.88 }        \\
\midrule
% \hdashline 
Single      & $\methodname_{\text{Llama2}}$             & 0.44      & \textbf{0.63}           & 0.90          \\
Multiple       & $\methodname_{\text{Llama2}}$             & \textbf{0.71}      & \textbf{0.64}           & \textbf{0.94}         \\
\bottomrule
\end{tabular}
}



\caption{Ablation study comparing single versus multiple alternate generations across different methods. Results are reported on the 10\% split of the TOFU. The best results are highlighted in \textbf{bold}.}

\label{multi_sub}
\end{table}
